iGVLM: Dynamic Instruction-Guided Vision Encoding for Question-Aware Multimodal Understanding

Despite the success of Large Vision--Language Models (LVLMs), most existing architectures suffer from a representation bottleneck: they rely on static, instruction-agnostic vision encoders whose visual representations are utilized in an invariant manner across different textual tasks. This rigidity hinders fine-grained reasoning where task-specific visual cues are critical. To address this issue, we propose iGVLM, a general framework for instruction-guided visual modulation. iGVLM introduces a decoupled dual-branch architecture: a frozen representation branch that preserves task-agnostic visual representations learned during pre-training, and a dynamic conditioning branch that performs affine feature modulation via Adaptive Layer Normalization (AdaLN). This design enables a smooth transition from general-purpose perception to instruction-aware reasoning while maintaining the structural integrity and stability of pre-trained visual priors. Beyond standard benchmarks, we introduce MM4, a controlled diagnostic probe for quantifying logical consistency under multi-query, multi-instruction settings. Extensive results show that iGVLM consistently enhances instruction sensitivity across diverse language backbones, offering a plug-and-play paradigm for bridging passive perception and active reasoning.

==> sec/origin_intro.tex <==
\section{Introduction}
\begin{figure}[t!]
\vskip 0.2in
  % \vspace{-0.1em}
\centering
\includegraphics[width=0.8\linewidth]{figure/visual.pdf}      
% \caption{\textbf{
% %Architectural differences in VLMs.
% Architectural Comparison of Vision-Language Models.} 
% Top: Pipeline of LLaVA-1.5.
% Middle: Pipeline of QA-ViT.
% Bottom: Pipeline of our proposed \textit{\name}. 
% %We employ a dual-branch to fuse pure vision features with instruction-guided features.
% Unlike prior approaches, \textit{\name} employs a dual-branch vision encoder that fuses static visual features with dynamically modulated, instruction-guided features for enhanced instruction-aware perception.
% }
\caption{\textbf{Qualitative visualization of instruction-conditioned feature utilization.}
We use Grad-CAM to qualitatively visualize the feature responses of the two vision branches in iGVLM under different textual instructions.
While the static branch exhibits largely invariant activation patterns, the instruction-guided branch shows instruction-dependent emphasis on task-relevant regions.
This visualization provides an intuitive illustration of how instruction-conditioned modulation can influence the utilization of visual features.}
\label{fig:visualization}
\vspace{-2em}
\end{figure}

In recent years, advances in computer vision~\cite{,DBLP:conf/cvpr/ZhangL0024,DBLP:conf/iccv/LiuL00W0LG21} and natural language processing~\cite{DBLP:conf/nips/VaswaniSPUJGKP17,radford2019language,brown2020language} have driven remarkable progress in Vision-Language Models (VLMs)~\cite{sharegpt4v,DBLP:journals/corr/abs-2403-05525,DBLP:journals/corr/abs-2312-14238,DBLP:journals/corr/abs-2401-04088}.  
By jointly modeling vision and language, these systems enable more comprehensive cross-modal understanding and have achieved strong performance on tasks such as image captioning, visual question answering, and grounded dialogue.  
This synergy between modalities marks a key step toward general-purpose multimodal intelligence.  
However, aligning visual perception with task-specific linguistic instructions remains an open challenge.


This challenge stems largely from the fact that most existing VLMs still rely on \textit{static, instruction-agnostic} vision encoders such as CLIP-ViT~\cite{DBLP:conf/icml/RadfordKHRGASAM21}, which extract visual features independently of task-specific instructions or user intent. 
As a result, these models are unable to adjust their visual attention based on the semantics of the given query, leading to suboptimal fine-grained reasoning and question-aware visual grounding (as illustrated in~\cref{fig:visualization}). 
Retraining vision encoders from scratch with instruction-conditioned objectives could introduce adaptability, but the process is prohibitively costly in computation and data, making it impractical for large-scale systems.
A more practical and scalable alternative is to augment existing vision encoders with lightweight, modular adaptation mechanisms that endow them with instruction-following capabilities without retraining from scratch.


%##################################################################################################
\begin{figure*}[t]\centering
\includegraphics[width=0.9\linewidth]{figure/convit.pdf}
    \caption{\textbf{(a): The proposed \name architecture.} The Text Encoder extracts features from the input instructions to guide the Vision Encoder, %dynamically adjusting the visual features. 
    enabling dynamic modulation of visual representations.
    These instruction-conditioned features are then fused with static visual features. 
    The fused representation is aligned with a Large Language Model (LLM) to generate responses. 
    The illustrated example comes from a real-world VQA scenario rather than the MM4 benchmark. 
    \textbf{(b): AdaLN-Modified ViT.} We leverage textual information to modulate the multi-head attention and MLP modules within the ViT the AdaLN adapter, %thereby directing the evolution of visual focus.
    enabling instruction-aware adjustment of visual attention.
}
\label{fig:mechanisms}
\vspace{-1em}
\end{figure*}
%##################################################################################################

% %Currently, two representative approaches aim to enable dynamic modulation of visual features based on user instructions: QA-ViT~\cite{DBLP:conf/cvpr/GanzKABNML24} and DyFo.
% Recent approaches have attempted to address this limitation by enabling dynamic visual feature modulation guided by text. Notably, 
% QA-ViT~\cite{DBLP:conf/cvpr/GanzKABNML24} injects textual representations into the %final third of a vision transformer while keeping most vision layers frozen. As a result, QA-ViT neither retains the complete static perceptual capabilities nor fully exploits the model’s potential to follow instruction-driven modulation.
% upper layers of a frozen vision transformer, introducing some instruction-awareness. However, this method neither fully retains static visual priors nor fully exploits the potential of dynamic visual adaptation. 
% On the other hand, DyFo~\cite{dyfo} employs an external expert model  (e.g., Lang-Segment-Anything~\cite{langsam}) combined with Monte Carlo Tree Search (MCTS) to simulate human-like attention shifts by selecting relevant regions to query.  While effective, DyFo's performance is heavily dependent on the external expert's quality and incurs high inference costs due to repeated model queries during MCTS. 

% We argue that an effective question-aware vision encoder should retain the  strong visual perception %and exhibit adaptive behavior under textual guidance. 
% capabilities of pretrained models while enabling adaptive visual modulation based on textual instructions. 
% Modern vision transformers already possess robust perceptual representations, and the core challenge lies in enhancing them  with flexible, instruction-conditioned adaptability without sacrificing perceptual fidelity.

To the best of our knowledge, several recent works have begun addressing this issue by introducing dynamic modulation mechanisms. 
QA-ViT~\cite{DBLP:conf/cvpr/GanzKABNML24} injects textual representations into the upper layers of a frozen vision transformer, introducing limited instruction awareness. 
While this design enables modest adaptability, it partially compromises the pretrained visual priors and fails to achieve robust instruction-conditioned modulation. 
In contrast, DyFo~\cite{dyfo} relies on an external expert model (e.g., Lang-Segment-Anything~\cite{langsam}) coupled with Monte Carlo Tree Search (MCTS) to simulate human-like attention shifts. 
Although effective, its performance heavily depends on the quality of the external expert and incurs substantial inference cost due to repeated model queries during the search process.

These limitations suggest that an effective question-aware vision encoder should preserve the strong perceptual capability of pretrained models while enabling flexible, instruction-conditioned adaptation. Modern vision transformers already provide strong perceptual representations. The key challenge is to endow them with dynamic, text-conditioned adaptability without compromising perceptual fidelity.


% To this end, we propose \textbf{iGVLM}, a novel \textbf{i}nstruction-\textbf{G}uided visual encoder for \textbf{V}ision-\textbf{L}anguage \textbf{M}odels. 
% iGVLM introduces a dual-branch architecture that decouples static and dynamic perception pathways. 
% The static branch retains a frozen pre-trained vision encoder to preserve task-agnostic visual priors, while the dynamic branch incorporates lightweight, instruction-conditioned adapter modules into the same backbone, enabling dynamic modulation of attention guided by text.  
% %to modulate attention maps based on instruction embeddings. 
% As illustrated in~\Cref{fig:mechanisms}(a), this architecture offers a modular and extensible %alternative to prior VLMs (DyFo does not modify the architecture of the VLM). 
% framework that enhances instruction-following capacity without compromising perceptual fidelity. 
% Unlike DyFo, which remains externally dependent and computationally costly, iGVLM provides a native, architecture-aware solution.

% We evaluate iGVLM on MMStar~\cite{DBLP:conf/emnlp/LiDZWZW23}, a comprehensive  benchmark focused on fine-grained multimodal reasoning. Experimental results show that iGVLM consistently outperforms existing dynamic modulation approaches across multiple reasoning tasks, while also yielding performance gains on standard general-purpose benchmarks. 
% Furthermore, we introduce MM4, the first benchmark specifically designed to assess the question-aware capabilities of VLMs. MM4 challenges models to answer multiple, diverse questions grounded in a single image,  providing a rigorous and realistic assessment of instruction-following behavior in multimodal contexts. We envision MM4 as a complementary benchmark to existing datasets% and hope it serves as a challenging and realistic standard to guide the development of next-generation VLMs.
% , serving as a more discriminative standard for next-generation VLMs. 

% Our contributions are summarized as follows:
% \begin{itemize}
%     \item We propose iGVLM, a novel instruction-guided vision encoder for VLMs%, which integrates a dual-branch architecture combining static and dynamic pathways. The static branch preserves pre-trained visual priors, while the dynamic branch injects lightweight, text-conditioned adapters to enable fine-grained, instruction-aware modulation of visual representations.
%     . It features a dual-branch architecture that combines a frozen static branch with a dynamic branch enhanced by lightweight, text-conditioned adapters for instruction-aware visual modulation.
%     \item We introduce MM4, the first benchmark explicitly designed to evaluate the question-aware visual perception. %, which challenges models to answer multiple diverse questions grounded on a single image. MM4 provides a rigorous and comprehensive protocol to assess instruction-following ability in multimodal settings.
%     It tasks models with answering multiple semantically diverse questions based on a single image, enabling a comprehensive and fine-grained evaluation of instruction-following abilities.
%     \item We conduct extensive experiments on MMStar and other standard multimodal benchmarks, demonstrating that iGVLM significantly outperforms existing dynamic modulation models in fine-grained reasoning tasks, while also improving performance on general-purpose %evaluation datasets.
%     multimodal evaluations. 
% \end{itemize}


To this end, we propose \textbf{iGVLM}, a novel \textit{instruction-guided} vision encoder for Vision-Language Models. 
iGVLM adopts a dual-branch architecture that decouples static and dynamic perception pathways. 
The static branch retains a frozen pre-trained vision encoder to preserve task-agnostic visual priors, 
while the dynamic branch integrates lightweight, instruction-conditioned adapter modules that modulate visual attention under textual guidance. 
% This design enables flexible, instruction-aware perception without retraining the backbone, achieving a balance between stability and adaptability. 
This design achieves flexible, instruction-aware perception without retraining, balancing stability and adaptability.
Unlike DyFo, which depends on external expert models and incurs heavy computational cost, iGVLM provides an efficient, architecture-aware solution for dynamic visual modulation.

We comprehensively evaluate iGVLM on the MMStar~\cite{DBLP:conf/nips/ChenLDZZCDWQLZ24} benchmark for fine-grained multimodal reasoning, 
where it consistently surpasses prior dynamic modulation approaches across multiple tasks while maintaining strong general multimodal performance. 
Furthermore, we introduce \textbf{MM4}, the first benchmark specifically designed to assess the \textit{question-aware} capabilities of VLMs. 
MM4 challenges models to answer multiple, semantically diverse questions grounded in a single image, 
offering a rigorous and realistic evaluation of instruction-following behavior in multimodal contexts. 

Our main contributions are as follows:
\begin{itemize}
    \item We propose \textbf{iGVLM}, a novel instruction-guided vision encoder featuring a dual-branch architecture that combines a frozen static branch with a dynamic branch augmented by lightweight, text-conditioned adapters for instruction-aware visual modulation.
    \item We introduce \textbf{MM4}, the first benchmark explicitly designed to evaluate question-aware visual perception by requiring models to answer diverse queries grounded in a single image.
    \item We conduct extensive experiments on MMStar and other multimodal benchmarks, demonstrating that iGVLM achieves state-of-the-art fine-grained reasoning performance while maintaining efficiency and general multimodal capability.
\end{itemize}


